Generative Knowledge Selection for Knowledge-Grounded Dialogues

Knowledge selection is the key in knowledge-grounded dialogues (KGD), which aims to select an appropriate knowledge snippet to be used in the utterance based on dialogue history. Previous studies mainly employ the classification approach to classify each candidate snippet as "relevant" or "irrelevant" independently. However, such approaches neglect the interactions between snippets, leading to difficulties in inferring the meaning of snippets. Moreover, they lack modeling of the discourse structure of dialogue-knowledge interactions. We propose a simple yet effective generative approach for knowledge selection, called GenKS. GenKS learns to select snippets by generating their identifiers with a sequence-to-sequence model. GenKS therefore captures intra-knowledge interaction inherently through attention mechanisms. Meanwhile, we devise a hyperlink mechanism to model the dialogue-knowledge interactions explicitly. We conduct experiments on three benchmark datasets, and verify GenKS achieves the best results on both knowledge selection and response generation.

==> tables/ablation-2.tex <==
\begin{table}[ht]
\centering
\small
\setlength\tabcolsep{4pt}
\begin{tabular}{@{}l cccc@{}}

\toprule
\multirow{2}{*}{}
% {\textbf{Methods}}
& \multicolumn{2}{c}{\textbf{WOW}} 
& \multicolumn{2}{c}{\textbf{Holl-E}}\\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
{} & \textbf{Seen} & \textbf{Unseen} & \textbf{Single} & \textbf{Multi} \\
\midrule
\textbf{GenKS} & 34.7  & 37.5 & 37.9 & 47.2\\
\midrule
{-~BART classification model} & 29.9 & 28.3 & 35.8 & 45.8\\
{-~Shuffle knowledge context} & 30.3 & 30.2 & 36.1 & 46.1\\
{-~Shuffle knowledge identifiers} & 31.3 & 32.5 & 36.5 & 46.9\\
{-~Use document FID model} & 14.6 & 22.1 & 14.7 & 22.4 \\
{-~Remove historical IDs} & 32.9 & 35.2 & 37.1 & 46.5\\
{-~Use the oracle passage} & 45.2 & 45.9 & 50.5 & 57.3\\
% \bottomrule
% \toprule
% \multirow{2}{*}{\textbf{(2) Response Generation}}
% % {\textbf{Methods}}
% & \multicolumn{2}{c}{\textbf{Seen}} 
% & \multicolumn{2}{c}{\textbf{Unseen}}\\
% \cmidrule(lr){2-3} \cmidrule(lr){4-5}
% & PPL & F1 & PPL & F1\\
% \midrule
% Base model & 14.2  & 22.1 & 14.7 & 22.3 \\
% \midrule
% % {-~Random selected knowledge} & 16.6 & 17.0 & 17.3 & 16.7 \\
% {-~Use KnowledGPT's knowledge} & 14.9 & 22.0 & 15.6 & 21.1 \\
% {-~Use two-stage model} & 14.6 & 22.1 & 14.7 & 22.4 \\
% {-~Use the oracle knowledge} & 8.9 & 37.5 & 9.5 & 37.9\\
\bottomrule
\end{tabular}
\caption{Ablation study about knowledge selection.
% The base model (\textsc{GenKS}) is compared with several variants. Part (1) gives evaluation results of knowledge selection on Wizard Seen, Wizard Unseen, Holl-E Single, and Holl-E Multi; See Section \ref{sec:ablation} for details. Part (2) gives evaluation results of response generation on Wizard; See Section \ref{sec:ablation-gen} for details.
}
\label{table:ablation}
\end{table}


==> tables/ablation-gen.tex <==
\begin{table}[!t]
\centering
\small
\setlength\tabcolsep{3pt}
\begin{tabular}{l cccc}

\toprule
\multirow{2}{*}{\textbf{Methods}}
% {\textbf{Methods}}
& \multicolumn{2}{c}{\textbf{Test Seen}} 
& \multicolumn{2}{c}{\textbf{Test Unseen}}\\
& PPL & F1 & PPL & F1\\
\hline
Baseline & 14.6  & 22.1 & 14.7 & 22.3 \\
\hline
{-~Random selected knowledge} & 30.3 & 31.3 \\
{-~Rank in order} & 30.3 & 32.5 \\
{-~Use BART-large} & 12.9 & 22.7 & 13.1 & 32.5 \\
{-~Use the oracle knowledge} & 43.8 & 45.5 \\
\bottomrule
\end{tabular}
\caption{Ablation studies of response generation on Wizard of Wikipedia. The baseline model is compared with several variants. See Section \ref{sec:ablation-gen} for detials.}
\label{table:ablation-gen}
\end{table}


==> tables/ablation.tex <==
\begin{table}[!t]
\centering
\small
\setlength\tabcolsep{3pt}
\begin{tabular}{l ccc}

\toprule
{} & \textbf{Seen} & \textbf{Unseen} & \textbf{Holl-E} \\
\hline
Baseline & 33.4  & 36.4 & 34.6\\
\hline
{-~Shuffle knowledge context} & 30.3 & 31.3 \\
{-~Remove tag in dialogue context} & 32.9 & 35.2 \\
{-~Shuffle knowledge tags} & 30.3 & 32.5 \\
{-~Use the oracle passage} & 43.8 & 45.5 \\
\bottomrule
\end{tabular}
\caption{Ablation studies of knowledge selection. The baseline model is compared with several variants. See Section \ref{sec:ablation} for detials.}
\label{table:ablation}
\end{table}


==> tables/gen-2.tex <==
\begin{table*}[!t]
\centering
\small
\setlength\tabcolsep{4pt}
\begin{tabular}{@{}l ccc ccc cccc cccc@{}}

\toprule
% \hline
\multirow{2}{*}{\textbf{Methods}}
% {\textbf{Methods}}
& \multicolumn{3}{c}{\textbf{WOW Seen}} 
& \multicolumn{3}{c}{\textbf{WOW Unseen}}
& \multicolumn{4}{c}{\textbf{Holl-E Single}}
& \multicolumn{4}{c}{\textbf{Holl-E Multi}}
\\
% \cline{2-11}
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-11} \cmidrule(lr){12-15}

{} & PPL & F1 & B4 & PPL & F1 & B4 & F1 & B4 & RG1 & RG2 & F1 & B4 & RG1 & RG2 \\

\midrule

% BART~\citep{} 
% & 14.7 & 20.9 & 1.7 
% & 18.9 & 18.7 & 0.9
% \\
% GPT-2~\citep{} 
% & 15.0 & 14.4 & 1.0
% & 18.9 & 13.8 & 0.8
% \\
% \hline

TMN~\citep{Dinan2019WizardOW}
& 66.5 & 16.9 & 0.4
& 97.3 & 14.3 & 0.3
& - & 6.7 & 28.2 & 10.0
& - & 8.9 & 32.5 & 13.1
\\
DukeNet~\citep{Meng2020DukeNetAD}
& 48.3 & 19.3 & 2.4
& 69.4 & 17.1 & 1.7 
& 30.5 & 19.2 & 36.5 & 23.0
& 37.6 & 26.8 & 43.2 & 30.1
\\
MIKe~\citep{Meng2021InitiativeAwareSL}
& 38.4  & 19.7  & 2.8
& 51.2 & 17.2 & 1.9
& \underline{32.1} & \underline{21.1} & \textbf{38.0} & 25.2
& \underline{38.3} & \underline{28.1} & \underline{44.1} & \underline{31.5}
\\
CoLV~\citep{Zhan2021CoLVAC}
& 39.5  & 20.3 & 2.8
& 54.3 & 18.5 & 2.1
& - & 20.3 & 32.0 & \underline{25.8}
& - & - & - & -
\\
KnowledGPT~\citep{Zhao2020KnowledgeGroundedDG}
& 19.2  & \underline{22.0} & \underline{3.7}
& 22.3 & \underline{20.5} & \underline{3.0}
& - & - & - & -
& - & - & - & -
\\
K-Mine~\citep{Lotfi2021TeachMW}
& 16.3 & 20.9 & - 
& 20.3 & 20.1 & -
& - & - & 36.1 & -
& - & - & - & -
\\
Graph~\citep{Li2022EnhancingKS}
& - & - & - 
& - & - & -
& - & - & 42.5 & 34.4
& - & - & 47.9 & 39.6
\\

\midrule

% \textbf{GenKS 2SG} 
% & 14.6 & \textbf{22.1} & \textbf{4.0} 
% & 14.7 & \textbf{22.4} & \textbf{4.6}
% % & \textbf{34.70} & \textbf{22.33}
% % & - & -
% % & - & -
% \\

\textbf{GenKS} 
& 14.2 & \textbf{22.1} & \textbf{3.9}
& 14.6 & \textbf{22.3} & \textbf{4.3}
& \textbf{32.7} & \textbf{22.3} & \textbf{38.0} & \textbf{27.9}
& \textbf{39.5} & \textbf{29.7} & \textbf{44.9} & \textbf{34.4}
\\

\bottomrule
\end{tabular}
\caption{Evaluation results on Wizard and Holl-E in terms of response quality. 
PPL denotes perplexity; B4 denotes BLEU-4; RG1 and RG2 denote ROUGE-1 and ROUGE-2, respectively.
The best results are highlighted with \textbf{bold}, and the second-best results are highlighted with \underline{underline}. 
PPL is not labeled in bold because the models with different vocabulary are not directly comparable.}
\label{table:gen}
\end{table*}


==> tables/gen.tex <==
\begin{table}[!t]
\centering
\small
\setlength\tabcolsep{3pt}
\begin{tabular}{l ccc ccc}

\toprule
% \hline
\multirow{2}{*}{\textbf{Methods}}
% {\textbf{Methods}}
& \multicolumn{3}{c}{\textbf{Test Seen}} 
& \multicolumn{3}{c}{\textbf{Test Unseen}}
\\
% \cline{2-11}
\cmidrule(lr){2-4} \cmidrule(lr){5-7}

{} & PPL & F1 & B4 & PPL & F1 & B4\\

\hline

TMN
& 66.5 & 15.9 & 0.4
& 103.6 & 14.3 & 0.3
\\
DukeNet 
& 48.3 & 19.3 & 2.4
& 69.4 & 17.1 & 1.7 
\\
CoLV 
& 39.5  & 20.3 & 2.8
& 54.3 & 18.5 & 2.1
\\
KnowledGPT
& 19.2  & 22.0 & 3.7
& 22.3 & 20.5 & 3.0
\\
MIKe
& 38.4  & 19.7  & 2.8
& 51.2 & 17.2 & 1.9
\\
K-Mine
& 16.3 & 20.9 & - 
& 20.3 & 20.1 & -
\\
\hline

% \textbf{GenKS 2SG} 
% & 14.6 & \textbf{22.1} & \textbf{4.0} 
% & 14.7 & \textbf{22.4} & \textbf{4.6}
% % & \textbf{34.70} & \textbf{22.33}
% % & - & -
% % & - & -
% \\

\textbf{GenKS} 
& \textbf{14.2} & \textbf{22.1} & \textbf{3.9}
& \textbf{14.6} & \textbf{22.3} & \textbf{4.3}
% & \textbf{34.70} & \textbf{22.33}
% & - & -
% & - & -
\\

\bottomrule
\end{tabular}
\caption{Results on Wikipedia of Wikipedia (Wizard) in term of response quality. PPL denotes perplecity, B4 denotes BLEU-4. GenKS 2SG and E2E represent GenKS Two-Stage and End-to-End respectively. The best results are highlighted with \textbf{bold}.}
\label{table:gen}
\end{table}


==> tables/speed.tex <==
\begin{table}[!t]
\centering
\small \setlength\tabcolsep{3pt}
\begin{tabular}{@{}l | cc | cc@{}}

\toprule
% \cline{2-11}
{} & KS & RG & ACC & F1\\

\midrule

% BART~\citep{Lewis2020BARTDS}
% & 0 & 5.2 
% & - & 18.9
% \\
BART RAG~\citep{Adolphs2021ReasonFT}
& 0 & 11.5
& - & 21.5
\\
BART FiD$^*$~\citep{Shuster2021RetrievalAR}
& 0 & 25.4
& - & 21.1
\\

\midrule
KnowGPT~\citep{Zhao2020KnowledgeGroundedDG}
& 12.5 & 7.4
& 25.4 & 20.5 
\\
K2R$^*$~\citep{Adolphs2021ReasonFT} 
& 11.8 & 8.2
& - & 19.9 
\\
% UniGDD~\citep{Adolphs2021ReasonFT} 
% & 12 & 11
% & - & 19.9 
% \\
DIALI$^*$~\citep{Li2022EnhancingKS} 
& 8.2 & -
& 35.5 & - 
\\
Graph$^*$~\citep{Li2022EnhancingKS} 
& 15.4 & -  
& 30.8 & - 
\\
\midrule

\textbf{GenKS}
& 2.9 & 8.8
& 36.6 & 22.9
\\
\bottomrule
\end{tabular}
\caption{Inference time (minutes) on one GPU on WoW
unseen test set. The values of model with $^*$ are estimated based on the model size and input/output length. KG and RG denote inference time for knowledge selection and response generation stage, respectively.}
\label{table:speed}
\end{table}

